Dynamic Queue-Jump Lane for Emergency Vehicles under Partially Connected Settings: A Multi-Agent Deep Reinforcement Learning Approach

Emergency vehicle (EMV) service is a key function of cities and is exceedingly challenging due to urban traffic congestion. The main reason behind EMV service delay is the lack of communication and cooperation between vehicles blocking EMVs. In this paper, we study the improvement of EMV service under V2X connectivity. We consider the establishment of dynamic queue jump lanes (DQJLs) based on real-time coordination of connected vehicles in the presence of non-connected human-driven vehicles. We develop a novel Markov decision process formulation for the DQJL coordination strategies, which explicitly accounts for the uncertainty of drivers' yielding pattern to approaching EMVs. Based on pairs of neural networks representing actors and critics for agent vehicles, we develop a multi-agent actor-critic deep reinforcement learning algorithm that handles a varying number of vehicles and a random proportion of connected vehicles in the traffic. Approaching the optimal coordination strategies via indirect and direct reinforcement learning, we present two schemata to address multi-agent reinforcement learning on this connected vehicle application. Both approaches are validated, on a micro-simulation testbed SUMO, to establish a DQJL fast and safely. Validation results reveal that, with DQJL coordination strategies, it saves up to 30% time for EMVs to pass a link-level intelligent urban roadway than the baseline scenario.

==> rl_dqjl.tex <==
% \subsection{Multi-agent actor-critic method}\label{subsec:multi_agent}
% With the success of actor-critic based learning algorithm in the control of the intelligent vehicle applications \cite{zhao2013supervised, nishi2019merging, yu2018intelligent, puccetti2019actor}, the actor-critic method is extended onto the multi-agent connected vehicle applications. In these connected vehicle applications, it is assumed, by the essential definition of multi-agent systems that each vehicle doesn't have the full knowledge of the road environment, but can partially observe its surroundings. The local observation contains information obtained through physical surroundings, such as neighboring vehicles' positions, as well as messages through communication channels among connected vehicles and the infrastructure. It is crucial to consider the compatibility of communication channels and message forms in the design the computing framework. Literature review introduces the following three actor-critic based learning frameworks in connected vehicle applications.

% \subsubsection{Fully centralized setting}
% In a fully centralize setting, all information is processed in a centralized controlled system. Namely, the policy and value networks for all vehicles, connected or autonomous, are stored in the centralized controller. At each step, all vehicles reports their own observation spaces to the controller and, as a result, the controller has the full knowledge of the road environment. The controller then perform decision makings after the reinforcement learning and send motion planning instructions to the corresponding vehicles. Under this setting, it is regarded that the centralized controller is operating as an "super-agent" to monitor and manage all connected agents. Many state-of-the-art ITS applications, such as \cite{zhao2013supervised, chen2020intelligent, su2020v2i}, are employing this framework to realize connected vehicle applications.

% The primary shortcoming of the fully centralized setting is its limitation usage. To have the full knowledge of the road environment, the centralized controller requires that all vehicles are connected, restricting its practicality within the short to medium future. The secondary concern of the framework regards with its high latency and synchronization cost, making real-time decision extremely difficult. The communication performance of the system may be bottle-necked by the vehicles of slowest message transmission, not to mention any potential data attack may result in the failure of the whole system.

% \subsubsection{Fully decentralized setting}
% In a fully decentralized setting, each vehicle has its own policy network and actor network deployed on board. Each vehicle interacts with the environment independently and a centralized controller, under this scheme, is no longer needed. Communications among vehicles are significantly reduced. Methodologies addressing the multi-agent vehicle applications under this setting are commonly referred as independent actor-critic (IAC) \cite{Tan93multi-agentreinforcement} method. Downgrading the multi-agent perspective to single-agent horizon, each vehicle's actor is updated based on its own state-action history. 

% Treating other vehicles as parts of the road environment, the fully decentralized setting faces huge risk of not converging becomes the environment becomes non-stationary. Depending on the application, the actor may not be able to make optimal decision for the vehicle at all. Secondly, due to no or minimal communication involved, each vehicle needs additional sensors, such as Lidar or cameras, to facilitate its perception about its surroundings. Such requirement for the agent vehicles significantly increases the cost of establishment of the framework. Lastly, vehicles in the decentralized setting are extremely non-resilient to stochastic road dynamics if their perception abilities are limited. They also have difficulties in identifying their roles in cooperative tasks.

% \subsubsection{Centralized training with decentralized execution}
% A more state-of-the-art multi-agent actor critic framework, proposed by \cite{lowe2017multiagent, foerster2017counterfactual}, adopts a new scheme of centralized training with decentralized execution. Under this framework, each vehicle has its own policy network deployed on board, while the corresponding value network is stored in the centralized controller. During the training stage, the centralized controller updates critic through TD learning with all agents' observation and their actions. The value network also takes in the immediate step reward to minimize the TD error elaborated in \eqref{eq:td_target}. The policy network, on the other hand, outputs the optimal action based on the vehicle's local observation. After the training stage, the value networks are completely abandoned and vehicles are able to operate based on their own observation spaces of the road environment and their policy networks.

% The centralized training with decentralized execution (CTDE) framework manages to overcome challenges in the previous settings. Since the centralized controller train value networks together, the road environment becomes stationary because the joint action is known, even though policy networks may change during the training stage. During the execution stage, vehicles have independent policy networks to guide them. Concerns regarding communication and synchronization costs are unnecessary during executions.

% Denoting the local observation and action for a vehicle as $o^{i}_{t}$ and $a^{i}_{t}$ at step $t$, the joint observation is then denoted as $\mathbf{o}_{t}$ and joint action as $\mathbf{a}_{t}$. The comparison between the three settings based on multi-agent actor critic method is shown in the Table. \ref{tab:marl_frameworks}.
% \begin{table}[]
% \centering
% \begin{tabular}{|c|c|c|c|c|}
% \hline
%  & Actor & Critic & Low Latency & Perception\\ \hline
% Centralized & $\pi(a^{i}_{t}|\mathbf{o}_{t}; \theta_{i})$ & $Q(\mathbf{o}_{t}, \mathbf{a}_{t};w_{i})$ & Required & Not required\\ \hline
% Decentralized & $\pi(a^{i}_{t}|o^{i}_{t}; \theta_{i})$  & $Q(o^{i}_{t}, a^{i}_{t};w_{i})$ & Not required & Required\\ \hline
% CTDE & $\pi(a^{i}_{t}|o^{i}_{t}; \theta_{i})$  &  $Q(\mathbf{o}_{t}, \mathbf{a}_{t};w_{i})$ & Not required & Not required\\ \hline
% \end{tabular}
% \caption{Multi-agent actor critic frameworks. The actors and critics, representing the policy networks and value networks respectively, indicate the input information are either local or global. Low latency shows their demand for low latency and synchronization cost during execution stage, while perception reveals if the framework needs Lidar/cameras when observing local environments.}
% \label{tab:marl_frameworks}
% \end{table}
% \FloatBarrier

